Toward Robust LiDAR based 3D Object Detection via Density-Aware Adaptive Thresholding

Robust 3D object detection is a core challenge for autonomous mobile systems in field robotics. To tackle this issue, many researchers have demonstrated improvements in 3D object detection performance in datasets. However, real-world urban scenarios with unstructured and dynamic situations can still lead to numerous false positives, posing a challenge for robust 3D object detection models. This paper presents a post-processing algorithm that dynamically adjusts object detection thresholds based on the distance from the ego-vehicle. 3D object detection models usually perform well in detecting nearby objects but may exhibit suboptimal performance for distant ones. While conventional perception algorithms typically employ a single threshold in post-processing, the proposed algorithm addresses this issue by employing adaptive thresholds based on the distance from the ego-vehicle, minimizing false negatives and reducing false positives in urban scenarios. The results show performance enhancements in 3D object detection models across a range of scenarios, not only in dynamic urban road conditions but also in scenarios involving adverse weather conditions.

==> fig_diff_fov_result.tex <==
\begin{figure*}[!t]
\begin{minipage}{.67\textwidth} %
  \centering
  \subfigure[Error Measured for Rotation (\textdegree) and Translation (\cm) Variation]{%
  \resizebox{0.92\textwidth}{!}{
  \begin{tabular}{c|cccc|c|ccccc}
    \toprule[1.5pt] % <-- Toprule here
    \midrule[0.5pt]
    Fixed & \multicolumn{4}{c|}{Rotation Variation (\textdegree)} &  Fixed & \multicolumn{5}{c} {Distance Variation (\cm)} \\
    Distance & 0$\rightarrow$20 & 20$\rightarrow$40 & 40$\rightarrow$60 & 60$\rightarrow$80 & Angle & 20$\rightarrow$25 & 25$\rightarrow$30 & 30$\rightarrow$35 & 35$\rightarrow$40 & 40$\rightarrow$45
    \\ \midrule[1pt]
    \unit{45}{cm} & 0.6398  & 0.0707 & 0.9675 & 1.2077 & 80\textdegree & 0.1697 & 0.1137 & 1.3918 &0.6780 & 1.3741 \\
    \unit{40}{cm} & 0.7586  & 0.1131 & 0.3187 & 0.2768 & 60\textdegree & 0.1584 & 1.0096 & 1.1799 & 1.3456 & 0.4132 \\
    \unit{35}{cm} & 0.1203  & 0.4511 & 0.8060 & 0.1947 & 40\textdegree & 0.3156 & 0.1831 & 0.7042 & 0.6292 & 0.5332 \\
    \unit{30}{cm} & 0.3974 & 0.2406 & 0.2435 & 0.3669 & 20\textdegree & 0.0120 & 0.0093 &0.3852 & 0.1017 & 0.1975 \\
    \unit{25}{cm} & 0.1790  & 0.1944 & 0.4898 & 0.1901 &  0\textdegree & 0.2690 & 0.2260 & 0.1161 & 0.1105 & 0.0595
    
    \\
    \unit{20}{cm} & 0.4953  & 0.4800 & 0.4810 & 1.1286 & & & & & & \\
   \midrule[0.5pt]
   \bottomrule[1pt]
   \end{tabular}
  }%resize 
  }
  
\end{minipage}%
\begin{minipage}{.37\textwidth} %
  \centering
  \subfigure[Error Heatmap]{%
    \includegraphics[height=0.12\textheight,width=0.9\columnwidth]{figures/heatmap.pdf}
    \label{fig:heatmap}
  }
\end{minipage}
\caption{Discrepancies between estimated pose variance and its actual value. As rotation and translation trend toward the top-right quadrant of the heatmap, error rates escalate. This elevation in error is primarily ascribed to a diminishing count of diverse feature matches as both cameras progressively capture different viewpoints.}
\label{fig:diff_fov}
\vspace{-0.3cm}
\end{figure*}


==> note.tex <==
# Free Notes


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \subfloat[Overlap of two images\label{fig:feature_overlap1}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap.png}
%     }
%     \subfloat[Revloution scan delay\label{fig:feature_overlap2}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap2.png}
% 	}\\
%     \subfloat[Contour and nearest point extraction\label{fig:feature_contour}]{
% 		\includegraphics[width=0.98\columnwidth]{./figs/features.pdf}
% 	}
%     \vspace{-1mm}
%     \caption{(a) In our dataset, certain regions remain un-updated due to the low update rate. An accumulation in these overlapping areas could lead to unexpected convergence behaviors. (b) Given that radar imagery inherently constitutes scan-rotated images, there exists a discrepancy between the commencement and conclusion of the scans, primarily attributed to temporal lags. This discrepancy is especially pronounced during sharp rotational movements. (c) Initially, we delineate the contour, subsequently identifying proximal points to ensure consideration extends beyond just the central points.}
%     \label{fig:feature}
%     \vspace{-5mm}
% \end{figure}


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \includegraphics[width=0.98\columnwidth]{./figs/fig3.pdf}
%     \vspace{-1mm}
%     \caption{Concept of the LodeStar Descriptor. From the primary radar imagery, we compute a radial intensity vector for every $\theta$. Each of these vectors is subsequently integrated to constitute a column within the integrated radial intensity matrix. By iterating this process over a period of 2$\pi$, we synthesize the final descriptor.}
%     \label{fig:lodestar}
%     \vspace{-5mm}
% \end{figure}


root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-48-03_minmax/recall_rates.csv 
STHEREO-SNU, 56.73, 74.61, 80.08, 84.90
STHEREO-valley, 83.60, 96.46, 98.71, 99.36
vivid-urban, 92.22, 98.13, 99.22, 99.69
vivid-city, 92.02, 96.55, 98.17, 98.99

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-49-24_histeq/recall_rates.csv 
STHEREO-SNU, 63.02, 79.35, 84.41, 88.33
STHEREO-valley, 75.88, 89.39, 94.53, 96.14
vivid-urban, 91.91, 98.29, 98.91, 99.69
vivid-city, 89.25, 97.84, 98.78, 99.19

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-50-31_minmax_gridwise_8x8/recall_rates.csv 
STHEREO-SNU, 53.55, 75.02, 81.31, 86.69
STHEREO-valley, 50.80, 71.38, 76.85, 81.99
vivid-urban, 88.49, 96.58, 98.76, 99.53
vivid-city, 91.62, 96.08, 97.50, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-51-45_minmax_gridwise_message_passing_8x8_mean_3/recall_rates.csv 
STHEREO-SNU, 61.80, 79.51, 85.22, 89.80
STHEREO-valley, 87.78, 97.43, 98.71, 99.04
vivid-urban, 93.78, 98.44, 99.07, 99.84
vivid-city, 92.97, 96.08, 97.57, 98.51

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-53-10_minmax_gridwise_message_passing_8x8_mean_5/recall_rates.csv 
STHEREO-SNU, 60.33, 77.80, 81.80, 87.27
STHEREO-valley, 90.03, 96.78, 98.07, 99.36
vivid-urban, 94.40, 99.22, 99.38, 99.84
vivid-city, 91.35, 96.42, 97.70, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-54-42_minmax_gridwise_message_passing_16x16_mean_3/recall_rates.csv 
STHEREO-SNU, 65.71, 80.24, 84.33, 89.06
STHEREO-valley, 76.21, 91.00, 95.18, 96.78
vivid-urban, 92.07, 97.51, 99.07, 100.00
vivid-city, 90.40, 96.35, 97.77, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-55-56_minmax_gridwise_message_passing_16x16_mean_5/recall_rates.csv 
STHEREO-SNU, 59.67, 77.55, 83.51, 88.24
STHEREO-valley, 76.85, 90.03, 95.50, 97.43
vivid-urban, 89.27, 97.20, 99.07, 99.84
vivid-city, 90.94, 95.47, 97.63, 98.58

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-57-11_minmax_gridwise_message_passing_16x16_mean_7/recall_rates.csv 
STHEREO-SNU, 60.90, 78.94, 84.90, 88.82
STHEREO-valley, 78.46, 93.89, 97.43, 99.36
vivid-urban, 90.82, 97.67, 99.38, 99.84
vivid-city, 90.80, 96.15, 97.90, 98.99

